Counter-Hypothetical Particle Filters for Single Object Pose Tracking

Particle filtering is a common technique for six degrees of freedom (6D) pose estimation due to its ability to tractably represent belief over object pose. However, the particle filter is prone to particle deprivation due to the high-dimensional nature of 6D pose. When particle deprivation occurs, it can cause mode collapse of the underlying belief distribution during importance sampling. If the region surrounding the true state suffers from mode collapse, recovering its belief is challenging since the area is no longer represented in the probability mass formed by the particles. Previous methods mitigate this problem by randomizing and resetting particles in the belief distribution, but determining the frequency of reinvigoration has relied on hand-tuning abstract heuristics. In this paper, we estimate the necessary reinvigoration rate at each time step by introducing a Counter-Hypothetical likelihood function, which is used alongside the standard likelihood. Inspired by the notions of plausibility and implausibility from Evidential Reasoning, the addition of our Counter-Hypothetical likelihood function assigns a level of doubt to each particle. The competing cumulative values of confidence and doubt across the particle set are used to estimate the level of failure within the filter, in order to determine the portion of particles to be reinvigorated. We demonstrate the effectiveness of our method on the rigid body object 6D pose tracking task.

==> Sections/Results/YCB_ADD_per_object.tex <==
\begin{table*}[]
\begin{tabular}{l|llllll|llllll|}
\cline{2-13}
 & \multicolumn{6}{c|}{\textbf{Single Frame Estimate}} & \multicolumn{6}{c|}{\textbf{Tracking}} \\ \hline
 \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Objects}}} & \multicolumn{2}{c|}{\textbf{PoseCNN}} & \multicolumn{2}{c|}{\textbf{DOPE}} & \multicolumn{2}{c|}{\textbf{CF PF}} & \multicolumn{2}{c|}{\textbf{PoseRBPF}} & \multicolumn{2}{c|}{\textbf{CF PF}} & \multicolumn{2}{c|}{\textbf{CF PoseRBPF}} \\ \cline{2-13} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{\textbf{ADD}} & \multicolumn{1}{l|}{\textbf{ADD-S}} & \multicolumn{1}{l|}{\textbf{ADD}} & \multicolumn{1}{l|}{\textbf{ADD-S}} & \multicolumn{1}{l|}{\textbf{ADD}} & \textbf{ADD-S} & \multicolumn{1}{l|}{\textbf{ADD}} & \multicolumn{1}{l|}{\textbf{ADD-S}} & \multicolumn{1}{l|}{\textbf{ADD}} & \multicolumn{1}{l|}{\textbf{ADD-S}} & \multicolumn{1}{l|}{\textbf{ADD}} & \textbf{ADD-S} \\ \hline
\multicolumn{1}{|l|}{\textbf{002\_master\_chef\_can}}& \multicolumn{1}{c|}{50.9} & \multicolumn{1}{c|}{84.0} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{36.6} & \multicolumn{1}{c|}{63.1} & \multicolumn{1}{c|}{47.0} & \multicolumn{1}{c|}{68.0} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{003\_cracker\_box}}& \multicolumn{1}{c|}{51.7} & \multicolumn{1}{c|}{76.9} & \multicolumn{1}{c|}{55.9} & \multicolumn{1}{c|}{69.8} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{74.2} & \multicolumn{1}{c|}{86.0} & \multicolumn{1}{c|}{61.2} & \multicolumn{1}{c|}{80.4} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{004\_sugar\_box}}& \multicolumn{1}{c|}{68.6} & \multicolumn{1}{c|}{84.3} & \multicolumn{1}{c|}{75.7} & \multicolumn{1}{c|}{87.1} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{75.4} & \multicolumn{1}{c|}{87.4} & \multicolumn{1}{c|}{70.0} & \multicolumn{1}{c|}{84.8} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{005\_tomato\_soup\_can}}& \multicolumn{1}{c|}{66.0} & \multicolumn{1}{c|}{80.9} & \multicolumn{1}{c|}{76.1} & \multicolumn{1}{c|}{85.1} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{69.0} & \multicolumn{1}{c|}{80.5} & \multicolumn{1}{c|}{58.5} & \multicolumn{1}{c|}{74.2} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{006\_mustard\_bottle}}& \multicolumn{1}{c|}{79.9} & \multicolumn{1}{c|}{90.2} & \multicolumn{1}{c|}{81.9} & \multicolumn{1}{c|}{90.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{23.7} & \multicolumn{1}{c|}{85.5} & \multicolumn{1}{c|}{51.7} & \multicolumn{1}{c|}{80.3} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{007\_tuna\_fish\_can}}& \multicolumn{1}{c|}{70.4} & \multicolumn{1}{c|}{87.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{53.4} & \multicolumn{1}{c|}{76.0} & \multicolumn{1}{c|}{35.7} & \multicolumn{1}{c|}{64.6} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{008\_pudding\_box}}& \multicolumn{1}{c|}{62.9} & \multicolumn{1}{c|}{79.0} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{63.6} & \multicolumn{1}{c|}{78.1} & \multicolumn{1}{c|}{36.4} & \multicolumn{1}{c|}{60.8} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{009\_gelatin\_box}}& \multicolumn{1}{c|}{75.2} & \multicolumn{1}{c|}{87.1} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{85.3} & \multicolumn{1}{c|}{90.8} & \multicolumn{1}{c|}{79.3} & \multicolumn{1}{c|}{89.2} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{010\_potted\_meat\_can}}& \multicolumn{1}{c|}{59.6} & \multicolumn{1}{c|}{78.5} & \multicolumn{1}{c|}{39.4} & \multicolumn{1}{c|}{52.4} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{19.4} & \multicolumn{1}{c|}{29.1} & \multicolumn{1}{c|}{34.4} & \multicolumn{1}{c|}{64.4} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{011\_banana}}& \multicolumn{1}{c|}{72.3} & \multicolumn{1}{c|}{85.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{27.3} & \multicolumn{1}{c|}{42.3} & \multicolumn{1}{c|}{24.3} & \multicolumn{1}{c|}{48.0} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{019\_pitcher\_base}}& \multicolumn{1}{c|}{52.5} & \multicolumn{1}{c|}{76.8} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{76.7} & \multicolumn{1}{c|}{88.3} & \multicolumn{1}{c|}{70.3} & \multicolumn{1}{c|}{86.0} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{021\_bleach\_cleanser}}& \multicolumn{1}{c|}{50.5} & \multicolumn{1}{c|}{71.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{48.1} & \multicolumn{1}{c|}{64.7} & \multicolumn{1}{c|}{30.3} & \multicolumn{1}{c|}{54.8} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{024\_bowl}}& \multicolumn{1}{c|}{6.5} & \multicolumn{1}{c|}{69.7} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{16.9} & \multicolumn{1}{c|}{86.0} & \multicolumn{1}{c|}{17.4} & \multicolumn{1}{c|}{80.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{025\_mug}}& \multicolumn{1}{c|}{57.7} & \multicolumn{1}{c|}{78.0} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{46.5} & \multicolumn{1}{c|}{77.1} & \multicolumn{1}{c|}{63.6} & \multicolumn{1}{c|}{83.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{035\_power\_drill}}& \multicolumn{1}{c|}{55.1} & \multicolumn{1}{c|}{72.8} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{64.3} & \multicolumn{1}{c|}{79.6} & \multicolumn{1}{c|}{60.1} & \multicolumn{1}{c|}{76.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{036\_wood\_block}}& \multicolumn{1}{c|}{31.8} & \multicolumn{1}{c|}{65.8} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{3.9} & \multicolumn{1}{c|}{22.4} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{037\_scissors}}& \multicolumn{1}{c|}{35.8} & \multicolumn{1}{c|}{56.2} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{26.6} & \multicolumn{1}{c|}{41.5} & \multicolumn{1}{c|}{28.1} & \multicolumn{1}{c|}{47.7} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{040\_large\_marker}}& \multicolumn{1}{c|}{58.0} & \multicolumn{1}{c|}{71.4} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{54.0} & \multicolumn{1}{c|}{61.9} & \multicolumn{1}{c|}{54.5} & \multicolumn{1}{c|}{63.7} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{051\_large\_clamp}}& \multicolumn{1}{c|}{25.0} & \multicolumn{1}{c|}{49.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{9.3} & \multicolumn{1}{c|}{30.3} & \multicolumn{1}{c|}{24.2} & \multicolumn{1}{c|}{40.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{052\_extra\_large\_clamp}}& \multicolumn{1}{c|}{15.8} & \multicolumn{1}{c|}{47.0} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{27.8} & \multicolumn{1}{c|}{67.6} & \multicolumn{1}{c|}{22.1} & \multicolumn{1}{c|}{46.0} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{061\_foam\_brick}}& \multicolumn{1}{c|}{40.4} & \multicolumn{1}{c|}{87.8} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{1.6} & \multicolumn{1}{c|}{5.9} & \multicolumn{1}{c|}{25.1} & \multicolumn{1}{c|}{55.3} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{|l|}{\textbf{ALL}}& \multicolumn{1}{c|}{53.7} & \multicolumn{1}{c|}{75.9} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{49.4} & \multicolumn{1}{c|}{69.0} & \multicolumn{1}{c|}{46.8} & \multicolumn{1}{c|}{68.3} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ \hline
\end{tabular}
\caption{\eo{Describe results}}
\label{table:results}
\end{table*}

==> Sections/Results/YCB_ADD_quantitative.tex <==
% \iffalse
% \begin{table*}[t]
% \centering
% \caption{\label{tab:ycb_quantitative} Quantitative results for the 6D pose tracking task on the YCB dataset. The metric is the area under the curve (AUC) for the average distance (ADD) and symmetric average distance (ADD-S) values for all parts.}
% \renewcommand{\arraystretch}{1.1}
% \begin{tabular}{r ccc ccc cc| ccc cc}
% \toprule
% % \multirow{2}{*}{\textbf{Object Set}}
% & \multicolumn{2}{c}{\textbf{PoseCNN}} && \multicolumn{2}{c}{\textbf{PoseRBPF}} && \multicolumn{2}{c}{\textbf{\methodabbr{} (Ours)}} & \multicolumn{2}{c}{\textbf{PoseRBPF}} && \multicolumn{2}{c}{\textbf{\methodabbr{} (Ours)}} \\ %\cline{2-11} 
% & &&& \multicolumn{2}{c}{\textbf{50 Particles}} && \multicolumn{2}{c}{\textbf{50 Particles}} & \multicolumn{2}{c}{\textbf{200 Particles}} && \multicolumn{2}{c}{\textbf{200 Particles}} \\
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{10-11} \cmidrule{13-14}
%  & ADD & ADD-S &&  ADD   & ADD-S && ADD   & ADD-S  & ADD   & ADD-S && ADD   & ADD-S  \\ 
% \midrule
% \textbf{Occluded} & 44.63  & 71.58   &&   47.28    &  73.16 && 42.63  &  65.40 &  52.61  &  68.34 && 51.81  &  69.77 \\ %\hline
% \textbf{Unoccluded} & 57.91     & 77.69      && 61.21  & 78.92    && 58.27 & 77.32    & 62.65  & 83.90  && 61.53   & 79.56\\ %\hline
% \textbf{ALL} & 53.10 & 75.48  && 55.80 & 76.67   && 55.20   & 72.69  & 59.32 & 78.62  && 58.31  & 76.47 \\ 
% \bottomrule
% \end{tabular}
% \end{table*}
% \fi

% START: OLD SINGLE RESULT TABLE
\begin{table*}[t]
\centering
\caption{\label{tab:quant} AUC scores for varying modifications of a 6D single object pose tracking particle filter on the YCB Video Dataset. Our presented method, CH-PF, outperforms other methods focused on alleviating particle deprivation in instances of occlusion, when the information from the likelihood function is the most accurate (RGB-D data).\eo{Jana, add more rows. Should we distinguish between 6D Particle filter and Rao-Blackwellized?}}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{r cc cc cc c cc cc cc}
\toprule
& \multicolumn{6}{c}{\bf RGB} && \multicolumn{6}{c}{\bf RGB-D}                                      
\\ \cmidrule{2-7} \cmidrule{9-14} 
& \multicolumn{2}{c}{Occluded} & \multicolumn{2}{c}{Non-Occluded}    & \multicolumn{2}{c}{All} && \multicolumn{2}{c}{Occluded} & \multicolumn{2}{c}{Non-Occluded}    & \multicolumn{2}{c}{All} 
\\ \cmidrule{2-7} \cmidrule{9-14} 
& {\footnotesize ADD}  & {\footnotesize ADD-S} & {\footnotesize ADD}  & {\footnotesize ADD-S} & {\footnotesize ADD}        & {\footnotesize ADD-S}    && {\footnotesize ADD}  & {\footnotesize ADD-S} & {\footnotesize ADD} & {\footnotesize ADD-S} & {\footnotesize ADD} & {\footnotesize ADD-S}     
\\\midrule
Annealing  & 40.0    & \multicolumn{1}{c|}{76.7}     & 55.5   & \multicolumn{1}{c|}{78.6}     & 48.7          & 77.7           && 47.8    & \multicolumn{1}{c|}{63.3}     & 77.0   & \multicolumn{1}{c|}{91.7}     & 64.2          & 79.2           \\
SRL        & 42.6    & \multicolumn{1}{c|}{\textbf{81.2}}     & 60.0   & \multicolumn{1}{c|}{79.1}     & 50.6          & 80.0           && 53.1    & \multicolumn{1}{c|}{81.3}     & 76.6  & \multicolumn{1}{c|}{92.1}     & 66.3          & 87.3           \\
Aug. MCL   & \textbf{44.7}    & \multicolumn{1}{c|}{80.6}     & 57.9   & \multicolumn{1}{c|}{78.9}     & 52.1          & 79.6           && 52.4    & \multicolumn{1}{c|}{78.2}     & \textbf{77.3}   & \multicolumn{1}{c|}{\textbf{92.3}}     & 66.4          & 86.1           \\
%Adapt. MCL & -    & \multicolumn{1}{c|}{-}     & -   & \multicolumn{1}{c|}{-}     & -          & -           & -    & \multicolumn{1}{c|}{-}     & -   & \multicolumn{1}{c|}{-}     & -          & -           \\
MCL + E2E     & 41.2    & \multicolumn{1}{c|}{62.3}     & \textbf{67.6}   & \multicolumn{1}{c|}{\textbf{87.7}}     & \textbf{56.0}          & 76.5           && 49.2    & \multicolumn{1}{c|}{65.4}     & 75.1   & \multicolumn{1}{c|}{92.0}     & 63.7          & 80.3           \\
CH-PF  (ours)    & 40.2    & \multicolumn{1}{c|}{80.9}     & 57.2   & \multicolumn{1}{c|}{81.4}     & 49.8          & \textbf{81.2}           && \textbf{59.3}   & \multicolumn{1}{c|}{\textbf{83.1}}     & 75.1   & \multicolumn{1}{c|}{92.2}     & \textbf{68.2}          & \textbf{88.2}           \\ 
\bottomrule
\end{tabular}
\end{table*}
% END: OLD SINGLE RESULT TABLE

% I am commenting this out because its hard to tell which I am editing - J
% \iffalse
% \begin{table*}[t]
% \centering
% \caption{\label{tab:ycb_quantitative} Quantitative results for the 6D pose tracking task on the YCB dataset. The metric is the area under the curve (AUC) for the average distance (ADD) and symmetric average distance (ADD-S) values for all parts.}
% \renewcommand{\arraystretch}{1.1}
% \begin{tabular}{r ccc ccc cc| ccc cc}
% \toprule
% % \multirow{2}{*}{\textbf{Object Set}}
% & \multicolumn{2}{c}{\textbf{PoseCNN}} && \multicolumn{2}{c}{\textbf{Standard}} && \multicolumn{2}{c}{\textbf{Counter-Hypothetical}} & \multicolumn{2}{c}{\textbf{Standard}} && \multicolumn{2}{c}{\textbf{Counter-Hypothetical}} \\ %\cline{2-11} 
% & &&& \multicolumn{2}{c}{\textbf{RBPF (3DoF)}} && \multicolumn{2}{c}{\textbf{RBPF (3DoF)}} & \multicolumn{2}{c}{\textbf{PF (6DoF)}} && \multicolumn{2}{c}{\textbf{PF (6DoF)}} \\
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{10-11} \cmidrule{13-14}
%  & ADD & ADD-S &&  ADD   & ADD-S && ADD   & ADD-S  & ADD   & ADD-S && ADD   & ADD-S  \\ 
% \midrule
% \textbf{Occluded} & -  & -   &&  -    &  - && -  &  - &  -  &  - && -  &  - \\ %\hline
% \textbf{Unoccluded} & -     & -      && -  & -    && - & -    & -  & -  && -   & -\\ %\hline
% \textbf{ALL} & - & -  && - & -  && -   & -  & - & -  && -  & - \\ 
% \bottomrule
% \end{tabular}
% \end{table*}
% \fi
